The Photographer Eye: Teaching Multimodal Large Language Models to Understand Image Aesthetics like Photographers

While editing directly from life, photographers have found it too difficult to see simultaneously both the blue and the sky. Photographer and curator, Szarkowski insightfully revealed one of the notable gaps between general and aesthetic visual understanding: while the former focuses on identifying the factual element in an image (sky), the latter transcends such object identification, viewing it instead as an aesthetic component--a pure color block (blue). Such fundamental distinctions between general (detection, localization, etc.) and aesthetic (color, lighting, composition, etc.) visual understanding present a significant challenge for Multimodal Large Language Models (MLLMs). Although some recent works have made initial explorations, they are often limited to general and basic aesthetic commonsense. As a result, they frequently fall short in real-world scenarios (Fig. 1), which require extensive expertise--including photographic techniques, photo pre/post-processing knowledge, and more, to provide a detailed analysis and description. To fundamentally enhance the aesthetics understanding of MLLMs, we first introduce a novel dataset, PhotoCritique, derived from extensive discussions among professional photographers and enthusiasts, and characterized by the large scale, expertise, and diversity. Then, to better learn visual aesthetics from PhotoCritique, we furthur propose a novel model, PhotoEye, featuring a languageguided multi-view vision fusion mechanism to understand image aesthetics from multiple perspectives. Finally, we present a novel benchmark, PhotoBench, a comprehensive and professional benchmark for aesthetic visual understanding. On existing benchmarks and PhotoBench, our model demonstrates clear advantages over existing models.

==> sec/5_benchmark.tex <==
% \section{Benchmarking Aesthetic Visual Understanding with Professionals}


% In Section 3, we highlighted a major limitation of existing datasets: annotations are typically provided by a few dozen number of annotators, which limits the diversity and expertise of the annotations. Even with reported training, these annotators lack the expertise of the many experienced photographers and enthusiasts. Existing benchmarks, such as Q-Bench~\cite{wu2024qbench} and AesBench~\cite{huang2024aesbench}, also suffer from this issue, relying on similar methods to obtain annotations. 

% To address the limitation and cover a wider range of scenarios, we directly draw insights from extensive photos and discussions on Reddit’s PhotoCritique, a vibrant community of photography professionals and enthusiasts.
% This approach allows us to generate comprehensive, diverse, and expert-level multiple-choice questions to evaluate the aesthetic visual understanding of MLLMs. Specifically, we do not generate MCQs from annotator-provided annotations; instead, we derive MCQs from photo reviews in Reddit’s PhotoCritique. We refer our new benchmark as \textbf{PhotoBench}. 
% Since RPCD~\cite{zhong2023aesthetically} has already collected raw comments from PhotoCritique posts between 2009 and 2022 alongside their corresponding photos, we directly design pipelines that use LLM (GPT-4-turbo) to generate MCQs.

% % \vspace{1.5mm}
% % \noindent \textbf{From Insights to Questions}

% \begin{figure*}[t]
% \vspace{-1mm}
% \centerline{\includegraphics[scale=0.24]{sec/img/bench.pdf}}
% \caption{We show one rejected example, several accepted examples, topic distribution, and some sub-topics of a subset of topics of questions in PhotoBench.}
% \label{fig:bench}
% % \vspace{-4mm}
% \end{figure*}



% \subsection{From Insights to Questions}
% The entire question generation process consists of three steps: (1) summarization, (2) question generation and (3) multi-stage filtering. 
% \textbf{(1) Summarization.} 
% Since the raw comments from the forum are quite noisy, empirically we find directly inputting the raw comments corresponding to an image to the LLM and prompting it to generate multiple-choice questions based grounded on these comments does not yield ideal results. To address this issue, we first use the LLM to summarize the noisy raw comments for each image, producing a single, clean, and comprehensive, and detailed photo critique. This process aligns with the pipeline shown in Fig.~\ref{fig:data_pipe}.
% %
% \textbf{(2) Question Generation.} For each image, we input its corresponding photo critique into the LLM and instruct it to generate five multiple-choice questions grounded on the provided critique.
% %
% \textbf{(3) Multi-stage Filtering.}
% This step directly impacts the quality of PhotoBench. We first selected the top 5,000 most detailed photo critiques from the initial generation step and instructed the LLM (using GPT-4 Turbo, as we empirically found it slightly outperforms GPT-4o) to generate 25,000 questions. 
% The first filtering stage is LLM-based, primarily aimed at removing MCQs with low visual dependency—that is, questions that could likely be answered correctly by reading only the question and options without viewing the image.We show an example in Fig.~\ref{fig:bench} (1). Our method is intuitive yet effective: we provide only the question and options to the LLM (GPT-4o) without the image and filter out questions it answers correctly. This step eliminated about 70\% of the items. We then instructed GPT-4o to score the remaining questions based on aesthetics relevance, visual dependency, and expertise. We selected the top 3,000 questions by average score and submitted them for review by experienced photographers, who further evaluated them against these standards. After this final review, we obtained 1,500 high-quality MCQs.
% \textcolor{red}{Details available in Appendix.}

% \subsection{PhotoBench} We show detailed information of PhotoBench in Fig.~\ref{fig:bench}. 
% Compared to existing works~\cite{wu2024qbench, huang2024aesbench, zhou2024uniaa}, Photobench gains more advantages in diversity and expertise. 
% %
% Due to potentially limited expertise and diversity among annotators~\cite{wu2024qbench, huang2024aesbench}, MCQs from existing works are often intuitive. We can have a straightforward comparison in Fig.~\ref{fig:bench_base}.
% %
% \begin{figure}[t]
% \vspace{-1mm}
% \centerline{\includegraphics[scale=0.27]{sec/img/bench_base.pdf}}
% \caption{Examples in related works from their original papers.}
% \label{fig:bench_base}
% \vspace{-4mm}
% \end{figure}
% %
% While questions from existing works are relatively straightforward and focus on factual elements, our questions are more challenging and practical, requiring \textbf{deeper aesthetics understanding} and covering topics \textbf{directly related to photography in practice}, such as camera settings, post-processing, and photographic techniques,  marked in blue in topics in Fig~\ref{fig:bench}.
% % example
% Examples are shown in Fig~\ref{fig:bench} (3,6). In Fig.~\ref{fig:bench} (3), to make the rainbow stand out more, the exposure should be reduced (slight underexposure can instead enhance color saturation). In Fig.~\ref{fig:bench} (6), we can observe that the shadows are not purely black but rather "grayish" (zoom in for a better view)—a common post-processing technique achieved by raising the shadow curve to enhance the photo’s texture or create a film-like aesthetic. They suggest that PhotoBench includes more professional and detailed questions, closely aligned with practical applications such as photo post-processing and editing.
% %


